On Single Index Models beyond Gaussian Data

Sparse high-dimensional functions have arisen as a rich framework to study the behavior of gradient-descent methods using shallow neural networks, showcasing their ability to perform feature learning beyond linear models. Amongst those functions, the simplest are single-index models $f(x) = \phi( x \cdot \theta^*)$, where the labels are generated by an arbitrary non-linear scalar link function $\phi$ applied to an unknown one-dimensional projection $\theta^*$ of the input data. By focusing on Gaussian data, several recent works have built a remarkable picture, where the so-called information exponent (related to the regularity of the link function) controls the required sample complexity. In essence, these tools exploit the stability and spherical symmetry of Gaussian distributions. In this work, building from the framework of \cite{arous2020online}, we explore extensions of this picture beyond the Gaussian setting, where both stability or symmetry might be violated. Focusing on the planted setting where $\phi$ is known, our main results establish that Stochastic Gradient Descent can efficiently recover the unknown direction $\theta^*$ in the high-dimensional regime, under assumptions that extend previous works \cite{yehudai2020learning,wu2022learning}.

==> scratch.tex <==


{\color{blue}

*** *** OLD *** *** 

\begin{theorem}[Gegenbauer to Hermite roots, regime $d \to \infty$, {\cite[Theorem 2]{f5277d02-ee90-3ae4-936b-eb33efe25beb}}] Let $z_{k,j,\lambda}$, $k=0,\ldots j$ be the zeros of $\bar{P}_{j,\lambda}$, and $h_{k,j}$, $k=0,\ldots j$ be the zeros of the Hermite polynomial $H_j$. Then, for each $j$,  
\begin{equation}
    z_{k,j,\lambda} = h_{k,j} \lambda^{-1/2} - \frac{h_{k,j}}{8} \left( 2j-1 + 2 h_{k,j}^2 \right) \lambda^{-3/2} + O(\lambda^{-5/2})~.
\end{equation}
\end{theorem}

\begin{theorem}[Location of Hermite roots, {\cite[Theorem 6.32]{szego1939orthogonal}}]
    Let $h_{j,j}$ and $h_{j-1,j}$ be respectively the largest and second largest root of $H_j$. Then there exists constants $C_1, C_2$ such that 
    \begin{equation}
        h_{k,j} = ( 2 j + 1)^{1/2} - C_k (2 j + 1)^{-1/6} + \epsilon_j ~,~ k \in \{j,j-1\}~,
    \end{equation}
    with $\epsilon_j = o( j^{-1/6})$. 
\end{theorem}



An immediate consequence of the fundamental theorem of calculus is 
\begin{lemma}
\begin{equation}
        \upsilon_{j,d} = \frac{j (j+d-2)}{d-1} \int_{{z}_{j-1,d+1}}^{{z}_{j,d}} P_{j-1,d+2}(t) dt~.
\end{equation}
\end{lemma}
Let us now use Lemma \ref{lem:basiccontrolgegen} to obtain simple bounds of $P_{j,d}(t)$ for $t \geq z_{j,d}$.
For each $\delta>0$, $j$ and $d$, let 
$$m(\delta, j, d) := | \{ z_{k,j,d} ; z_{k,j,d} \geq z_{j,d} - \delta \} |$$ 
denote the number of zeros of $P_{j,d}$ in the interval $(z_{j,d}-\delta, z_{j,d})$. 
We have
\begin{fact}
    \begin{equation}
        P_{j,d}(t) \leq \left(\frac{t^2 - (z_{j,d}-\delta)^2}{1-(z_{j,d}-\delta)^2} \right)^{m(\delta, j, d)}~.
    \end{equation}
\end{fact}



We collect several useful bounds for Gegenbauer polynomials, from \cite{szego1939orthogonal}. 
% \begin{theorem}[{\cite[Theorem 8.21.13]{szego1939orthogonal}}]
%     \begin{equation}
%         \bar{P}_{j, \lambda}(\cos \theta) = j^{-1/2} \pi^{-1/2} \left(\frac12 \sin \theta \right)^{-\lambda} \left\{ \cos((j + \lambda) \theta -\lambda \pi /2) + (j \sin(\theta))^{-1} O(1)\right\}
%     \end{equation} 
%     for $c j^{-1} \leq \theta \leq \pi - c j^{-1}$. %and where 
%    % $$K(\theta) = ~,~N = ~,~\gamma = ~.$$
% \end{theorem}

\begin{theorem}[{\cite[Theorem 8.21.12]{szego1939orthogonal}}]
\label{thm:besselgegen}
    \begin{equation}
        \bar{P}_{j, \lambda}(\cos \theta) = \left(\frac12 \sin \theta \right)^{-\lambda} \left( (j+\lambda)^{-\lambda+\frac12} \frac{\Gamma(j + \lambda + \frac12)}{j!}\sqrt{\frac{\theta}{\sin \theta}} J_{\lambda-1/2}((j+\lambda) \theta) + \theta^{1/2}O(j^{-3/2})\right)~,
    \end{equation}
    where $J_\nu(z)$ is the Bessel function of the first kind. 
\end{theorem}

\begin{theorem}[{\cite[Eq (3.4.5)]{gallardo}}]
    Let $\Lambda_\nu(x) = \frac{\Gamma(\nu+1) J_\nu(x)}{(\frac12 x)^\nu}$ and $N = j + \lambda + \frac12$. 
    We have
    \begin{equation}
        \left(\frac{\sin \theta}{\theta} \right)^{\lambda+\frac12} P_{j,2\lambda+2}(\cos \theta) = \Lambda_\lambda( N \theta) + R_j(\theta)~,
    \end{equation}
    where $R_j(\theta) = \theta^{\frac12 - \lambda} j^{-3/2-\lambda} O_j(1)$ for $C j^{-1} \leq \theta \leq \pi - \epsilon$, and $R_j(\theta) = \theta^2 O_j(1)$ for $0 \leq \theta \leq C j^{-1}$. 
\end{theorem}

% \begin{fact}
%     For $\cos \theta_{j,d} = z_{j-1,d+2}$, we have 
%     $$\left(\frac{\sin \theta_{j,d}}{\theta_{j,d}} \right)^{\lambda+\frac12} \geq $$
%     $$|\Lambda_\lambda(N \theta_{j,d})| \leq \kappa^{-\lambda} $$
%     $$|R_j(\theta_{j,d})| \leq B \kappa^{-\lambda}  $$
% \end{fact}

\begin{corollary}[Behavior of $\upsilon_{j,d}$, large $j$ regime] Assume the Ansatz $\left(\frac{\sin \theta}{\theta} \right)^{\lambda+\frac12} P_{j,2\lambda+2}(\cos \theta) \sim \Lambda_\lambda( N \theta)$. Then 
    \begin{equation}
        \upsilon_{j,d} \lesssim (e/2)^{-\lambda} \lambda^{1/6} \left[1 + \frac{\lambda^2}{j(j+2\lambda)} \right]^{\lambda + 1/2} ~.
    \end{equation}
    In particular, if $j > \lambda$, then there exists $\rho < 1$ such that 
    \begin{equation}
        \upsilon_{j,d} = O( \rho^{d} )~.
    \end{equation}
\end{corollary}
\begin{proof}
    The largest root of $P_{j,d}$ is given by Fact \ref{fact:largestroot}, by 
    $$z_{j,d}\leq \sqrt{\frac{(j-1)(j+d-4)}{(j+d/2-3)(j+d/2-2)}} \cos(\pi/(j+1)) := z_{j,d}^*~.$$

  Let $\cos \theta_{j,d} = z_{j-1,d+2}^*$.
From the Ansatz $\left(\frac{\sin \theta}{\theta} \right)^{\lambda+\frac12} P_{j,2\lambda+2}(\cos \theta) \sim \Lambda_\lambda( N \theta)$, and using Cauchy's asymptotic formula $J_\lambda(\lambda) \simeq \frac{\Gamma(1/3)}{2^{2/3} 3^{1/6} \pi \lambda^{1/3}}$ as well as Stirling's formula, we obtain
 \begin{align*}
    \upsilon_{j,\lambda} &= |P_{j,2\lambda+2}( \cos( \theta_{j, \lambda}) )| \\
    & \leq \left(\frac{\sin \theta_{j,d}}{\theta_{j,d}} \right)^{-\lambda-\frac12} 2^\lambda \lambda! J_\lambda\left( \theta_{j,d}(j+\lambda+1/2) \right) (\theta_{j,d}(j+\lambda+1/2))^{-\lambda} \\ 
    & \lesssim \left[\frac{(j+\lambda-2)(j+\lambda-1)}{(j-1)(j+2\lambda-2)} \right]^{\lambda + 1/2} 2^\lambda \lambda! J_\lambda( \sqrt{\lambda (\lambda-1)})  \lambda^{-\lambda} \\
    &\lesssim \left[\frac{(j+\lambda-2)(j+\lambda-1)}{(j-1)(j+2\lambda-2)} \right]^{\lambda + 1/2} \lambda^{-1/3-\lambda} 2^\lambda \lambda! \\
    & \lesssim (e/2)^{-\lambda} \lambda^{1/6} \left[1 + \frac{\lambda(\lambda-1)}{(j-1)(j+2\lambda-2)} \right]^{\lambda + 1/2}  
\end{align*}




% If we denote $C_d = \min_z J_{d/2}(z)$, and since $P_{j,\lambda}(z) > 0$ for $z > z_{j,d}$, 
% we thus have 
% \begin{align*}
%     \upsilon_{j,d} &\leq \frac{j! (d-3)!}{(j+d-3)!} \left(\frac{\sqrt{1-z_{j,d}^2}}{2}\right)^{-d/2} \left( (j+d/2)^{-d/2} \frac{\Gamma(j+d/2)}{j!} \sqrt{1-z_{j,d}^2}^{-1/2} C_{d} + O(j^{-3/2}) \right) \\
%     & = O( j^{-3d/4})~.
% \end{align*}
    
\end{proof}



\begin{lemma}%[{ \cite[Lemma 2.3]{de2008local}}]
Let $g_{j,d}$ be the gap between the largest and second largest root of $P_{j,d}$. For any $j \geq 2$, it holds  
    \begin{align}
        \upsilon_{j,d} &\leq \frac{j(j+d-2)}{d-1}  g_{j,d} z_{j,d}^{j-1}~.
    \end{align}
\end{lemma}
\begin{proof}
    The proof is a simple modification of the argument in \cite[Lemma 2.3]{de2008local}, in which we apply the mean-value theorem between consecutive zeros. 

Following \cite[Lemma 2.3]{de2008local}, we have that $\upsilon_{j,d} \leq \sup_{x \in [0, z_{j,d})} |P_{j,d}|$, where $z_{j,d}$ is the largest positive root of $P_{j,d}$. This maximum is attained at the largest root of $P'_{j,d} = \frac{j(j+d-2)}{d-1} P_{j-1,d+2}$, which by consistency we denote by $z_{j-1,d+2}$. 
%Let $\tilde{z}_{j,d}$ be the second-largest root of $P_{j,d}$, which by the interlacing property of orthogonal polynomials satisfies $\tilde{z}_{j,d} \leq z_{j-1,d+2}$. 
By the mean-value theorem, there exists $\zeta \in (z_{j-1,d+2}, z_{j,d})$ such that 
\begin{align*}
    P_{j,d}(z_{j-1,d+2}) - P_{j,d}( {z}_{j,d}) &= ( z_{j-1,d+2} - {z}_{j,d}) P_{j,d}'(\zeta)~,
\end{align*}
thus 
\begin{equation}
    \upsilon_{j,d} \leq ( z_{j,d} - {z}_{j-1,d+2}) \frac{j(j+d-2)}{d-1} \zeta^{j-1} \leq \frac{j(j+d-2)}{d-1} \cdot  z_{j,d}^j~,
\end{equation}
since $P_{j-1,d+2}(z) \leq z^{j-1}$ in $(z_{j-1,d+2}, 1]$. 
% By the mean-value theorem, there exists $\zeta \in (\tilde{z}_{j,d}, z_{j-1,d+2})$ such that 
% \begin{align*}
%     P_{j,d}(z_{j-1,d+2}) - P_{j,d}( \tilde{z}_{j,d}) &= ( z_{j-1,d+2} - \tilde{z}_{j,d}) P_{j,d}'(\zeta)~,
% \end{align*}
% thus 
% \begin{equation}
%     \upsilon_{j,d} \leq ( z_{j-1,d+2} - \tilde{z}_{j,d}) \frac{j(j+d-2)}{d-1} \upsilon_{j-1,d+2} \leq \frac{j(j+d-2)}{d-1} g_{j,d} \cdot  \upsilon_{j-1,d+2}~.
% \end{equation}
\end{proof}

Collecting the bounds so far, we have 
\begin{corollary}

    There exist sequences $(C_j)_j$, $(\tilde{C}_d)_d$ such that 
    \begin{equation}
        \upsilon_{j,d} \leq \min(1, C_j d^{-j/2}, \tilde{C}_d j^{-3d/4})~.
    \end{equation}
    $C_j$ can be explicitly bounded from the upper bounds on $z_{j,d}$. 
    $\tilde{C}_d$ remains unknown. 
\end{corollary}



\begin{fact}[Gegenbauer Representation in terms of Hermite]
\begin{equation}
    \bar{P}_{j,\lambda}(t) = ( \lambda(1-2t^2))^{j/2} \sum_{k=0}^j \frac{c_k}{z^k} \frac{H_{j-k}(\zeta)}{(j-k)!}~,
\end{equation}
where $\zeta = t \lambda / \sqrt{( \lambda(1-2t^2))}$ and the coefficients $c_k$ are the MacLaurin series of $f(t, w) = e^{-2 \lambda t w + \lambda(1-2t^2)w^2}(1-2tw + w^2)^{-\lambda}$. 
In particular, we have 
\begin{equation}
    P_{j,d}(t) \approx \frac{(d/2)^{j/2} (d-3)!}{(j+d-3)!} H_j( \sqrt{d/2} t)  ~.
\end{equation}
\end{fact}
\begin{corollary}
    \begin{equation}
        \upsilon_{j,d} \leq \frac{j! (d-3)!}{(j+d-3)!} \left( \frac{(d/2)^{j/2}}{j!} \min_t H_j(t) + O( d^{-\alpha} ) \right)
    \end{equation}
        \begin{equation}
        \upsilon_{j,d} \simeq \frac{ (d-3)!}{(j+d-3)!} (d/2)^{j/2} \min_t H_j(t) 
    \end{equation}
\end{corollary}


\begin{fact}
    Let $g_{j,d}$ be the gap between the largest and second largest root of $P_{j,d}$. Then for $d \geq 3$, 
    \begin{align}
        \upsilon_{j,d} &\leq \frac{j(j+d-2)}{d-1} g_{j,d} \cdot \upsilon_{j-1,d+2}~.
    \end{align}
\end{fact}
\begin{proof}
    The proof is a simple modification of the argument in \cite[Lemma 2.3]{de2008local}, in which we apply the mean-value theorem between consecutive zeros. 
    
Following \cite[Lemma 2.3]{de2008local}, we have that $\upsilon_{j,d} \leq \sup_{x \in [0, z_{j,d})} |P_{j,d}|$, where $z_{j,d}$ is the largest positive root of $P_{j,d}$. This maximum is attained at the largest root of $P'_{j,d} = \frac{j(j+d-2)}{d-1} P_{j-1,d+2}$, which by consistency we denote by $z_{j-1,d+2}$. Let $\tilde{z}_{j,d}$ be the second-largest root of $P_{j,d}$, which by the interlacing property of orthogonal polynomials satisfies $\tilde{z}_{j,d} \leq z_{j-1,d+2}$. By the mean-value theorem, there exists $\zeta \in (\tilde{z}_{j,d}, z_{j-1,d+2})$ such that 
\begin{align*}
    P_{j,d}(z_{j-1,d+2}) - P_{j,d}( \tilde{z}_{j,d}) &= ( z_{j-1,d+2} - \tilde{z}_{j,d}) P_{j,d}'(\zeta)~,
\end{align*}
thus 
\begin{equation}
    \upsilon_{j,d} \leq ( z_{j-1,d+2} - \tilde{z}_{j,d}) \frac{j(j+d-2)}{d-1} \upsilon_{j-1,d+2} \leq \frac{j(j+d-2)}{d-1} g_{j,d} \cdot  \upsilon_{j-1,d+2}~.
\end{equation}
    
\end{proof}

\begin{fact}[Gap between largest and second largest root of $P_{j,d}$, regime $j \leq d$]
\label{fact:gap_smallj}
We have the following control of $g_{j,d}$:
\begin{equation}
    g_{j,d} = O ( \sqrt{j/d} )~.
\end{equation}
Moreover, as $j, d \to \infty$, we have the refinement 
\begin{equation}
    g_{j,d} = C j^{-1/6} d^{-1/2} + O(d^{-3/2}) + o( j^{-1/6})~.
\end{equation}
\end{fact}
\begin{proof}
    We combine the asymptotic relation between Gegenbauer and Hermite zeroes from \cite[Theorem 2]{f5277d02-ee90-3ae4-936b-eb33efe25beb} and the location of Hermite zeros from \cite[Theorem 6.32]{szego1939orthogonal}.
\begin{theorem}[Gegenbauer to Hermite roots, {\cite[Theorem 2]{f5277d02-ee90-3ae4-936b-eb33efe25beb}}] Let $x_{j,k,\lambda}$, $k=0,\ldots j$ be the zeros of $\bar{P}_{j,\lambda}$, and $h_{j,k}$, $k=0,\ldots j$ be the zeros of the Hermite polynomial $H_j$. Then 
\begin{equation}
    x_{j,k,\lambda} = h_{j,k} \lambda^{-1/2} - \frac{h_{j,k}}{8} \left( 2j-1 + 2 h_{j,k}^2 \right) \lambda^{-3/2} + O(\lambda^{-5/2})~.
\end{equation}
\end{theorem}
\begin{proposition}[{\cite[Eq (6.31.19)]{szego1939orthogonal}}]
    Let $h_{j,1}$ and $h_{j,2}$ be respectively the largest and second largest root of $H_j$.
There exist constants $b, B$ such that 
\begin{equation}
    b\sqrt{j} \leq h_{j,2} < h_{j,1} \leq B \sqrt{j}.
\end{equation}
\end{proposition}
\begin{theorem}[Location of Hermite roots, {\cite[Theorem 6.32]{szego1939orthogonal}}]
    Let $h_{j,1}$ and $h_{j,2}$ be respectively the largest and second largest root of $H_j$. Then there exists constants $C_1, C_2$ such that 
    \begin{equation}
        h_{j,k} = ( 2 j + 1)^{1/2} - C_k (2 j + 1)^{-1/6} + \epsilon_j ~,~ k \in \{1,2\}~,
    \end{equation}
    with $\epsilon_j = o( j^{-1/6})$. 
\end{theorem}
\end{proof}
\begin{fact}[Gap $g_{j,d}$, regime $j \gg d$]
\label{fact:gap_largej}
In the regime $j \gg d$, we have 
    $g_{j,d} =  O\left( \frac{d^{4/3}}{j^2}\right)~.$
\end{fact}
\begin{proof}
    We first use the asymptotic expression of the zeros of Jacobi polynomials in terms of Bessel functions, given by 
    \begin{theorem}[{\cite[Theorem 8.12]{szego1939orthogonal}}]
        Let $x_{1n} > x_{2n} \dots $ be the zeros of $P_{n}^{(\alpha, \beta)}(x)$ in $[-1,+1]$ in decreasing order. If we write $x_{\nu n} = \cos(\theta_{\nu n})$, $0 < \theta_{\nu n} < \pi$, then for a fixed $\nu$, $\lim_n n \theta_{\nu n} = j_\nu$, where $j_\nu$ is the $\nu$-th positive zero of $J_\alpha(z)$. 
    \end{theorem}
    Now, from \cite[Section 7]{doi:10.1098/rsta.1954.0021} we use the asymptotic expression for the zeros of $J_{\lambda-1/2}$. As a result, if we let $x_{j,1,\lambda}, x_{j, 2, \lambda}$ be the two largest positive roots of $\bar{P}_{j,\lambda}$, then there exists two constants $B_1,B_2$ such that 
    \begin{equation}
        \arccos( x_{j,k,\lambda}) \simeq \frac{d}{2j} + B_k \frac{d^{1/3}}{j} + o(d^{1/3}/j)~,~k=1,2~.
    \end{equation}
    It follows that 
    \begin{align}
        g_{j,d} &= x_{j,1,\lambda} - x_{j, 2, \lambda} \nonumber \\
        &= \cos( \arccos( x_{j,1,\lambda} ) ) - \cos( \arccos( x_{j,2,\lambda} ) ) \nonumber \\
        &\simeq C \sin(d/2j) \frac{d^{1/3}}{j} \nonumber \\
        & = O\left( \frac{d^{4/3}}{j^2}\right)~.
    \end{align}
\end{proof}

\begin{fact}
    We have $\upsilon_{3, d} \simeq d^{-3/2}$.
\end{fact}
\begin{proof}
    Using the recurrence (\ref{eq:recurrgegen}) we directly obtain that 
    \begin{align*}
     2\bar{P}_{2, \lambda}(t) &= 2 ( 1 + \lambda) t \bar{P}_{1, \lambda}(t) - 2\lambda = 2\lambda( 2( 1 + \lambda) t^2 - 1) \\ %2 \lambda - 2\lambda\\
    3 \bar{P}_{3,\lambda}(t) &= 2( 2 + \lambda) t \bar{P}_{2, \lambda}(t) - (1 + 2\lambda) \bar{P}_{1,\lambda}(t) ~,  
    \end{align*}
    and thus 
    \begin{equation}
        \bar{P}_{3,\lambda}(t) = \frac{2 \lambda}{3} \left((2+ \lambda)t (2(1+\lambda)t^2 -1) - (1+2\lambda)t  \right)~.
    \end{equation}

    From the identity $\bar{P}'_{j, \lambda} = 2 \lambda \bar{P}_{j-1, \lambda+1}$ we deduce that the positive critical points of $\bar{P}_{3, \lambda}$ are given by $t^* = \sqrt{\frac{1}{2(2+\lambda)}}$, and therefore 
    \begin{align*}
        \upsilon_{3,d} & = \frac{\Gamma(4) \Gamma(d-2)}{\Gamma(d+1)} |\bar{P}_{3, \frac{d}{2}-1}(t^*) | \\
        &= \frac{6}{d (d-1) (d-2)} \frac{d-2}{3} \left| \frac{\sqrt{\frac{d}{2} + 1}}{\sqrt{2}} (d /(d+2) - 1) - \frac{d-1}{\sqrt{d+2}} \right| \\
        &= \frac{2}{d (d-1)} \left( \frac{1}{\sqrt{d+2}} + \frac{d-1}{\sqrt{d+2}} \right) \\
        &= \frac{2}{(d-1)\sqrt{d+2}}~.
    \end{align*}
\end{proof}
% \begin{corollary}

%     \begin{align}
%         \upsilon_{j,d} &\leq C \frac{j^{5/6} (j+d-2)}{d^{3/2}} \cdot \upsilon_{j-1,d+2}~,
%     \end{align}
%     with $\upsilon_{3, d} \simeq d^{-5/2}$. 
% \end{corollary}
Combining the previous facts, and relying on the asymptotic expressions from Facts \ref{fact:gap_smallj}, \ref{fact:gap_largej}
we arrive at 
\begin{corollary}
    We have, at leading order term, the bound
    % \begin{equation}
    %     \upsilon_{j,d} \leq \frac{C^j (j!)^{5/6} (2j+d-2)! ((d-1)!)^{3/2}}{(j+d-2)! ((d+2j)!)^{3/2} (d + 2j)^{3/2} }~.
    % \end{equation}
MIGHT not be strong enough.. look for a simpler route
\end{corollary}
\begin{proof}
    Assume first $j>d$. Let $\Delta = \lfloor(j-d)/3\rfloor$. We have 
\begin{align}
\label{eq:gup0}
    \upsilon_{j,d}& \leq C\frac{ (j+d-2) d^{1/3}}{j} \upsilon_{j-1,d+2}  \nonumber \\
    &\leq C^2 \frac{ (j+d-2)(j+d-1) (d (d+2))^{1/3}}{j(j-1)} \upsilon_{j-2,d+4} \nonumber  \\
    & \dots \nonumber  \\
    & \leq C^\Delta \frac{ (j+d-2)(j+d-1)\dots (j+d+\Delta-2) (d (d+2) \dots (d+2\Delta)^{1/3}}{j(j-1)\dots (j-\Delta)} \upsilon_{j-\Delta,d+2\Delta}~.
\end{align}
On the other hand, using now Fact \ref{fact:gap_smallj} we have 
\begin{align}
\label{eq:gup1}
    \upsilon_{j-\Delta,d+2\Delta} & \leq \tilde{C} \frac{(j-\Delta)^{5/6} (j+d+\Delta-2)}{(d+2\Delta)^{3/2}} \upsilon_{j-\Delta-1, d+2\Delta+2} \nonumber \\
    & \leq \tilde{C}^2  \frac{((j-\Delta)(j-\Delta-1))^{5/6} (j+d+\Delta-2)(j+d+\Delta-1)}{((d+2\Delta)(d+2\Delta+2))^{3/2}} \upsilon_{j-\Delta-2, d+2\Delta+4} \nonumber \\
    & \dots \nonumber \\
    & \leq \tilde{C}^{j -\Delta} \frac{(j!)^{5/6} \cdot (2j+d-2)! \cdot ((d+2\Delta)!!)^{3/2} }{ (j+d+\Delta-3)! \cdot ((d+2j)!!)^{3/2}} (d+2j)^{-3/2}
\end{align}
Putting together (\ref{eq:gup0}) and (\ref{eq:gup1}) we obtain
{\small
\begin{align}
    \upsilon_{j,d} &\leq \max(C, \tilde{C})^j (d+2j)^{-3/2} \frac{(j!)^{5/6} \cdot (2j+d-2)! \cdot ((d+2\Delta)!!)^{3/2} }{ (j+d+\Delta-3)! \cdot ((d+2j)!!)^{3/2}} \frac{ (j+d-2)(j+d-1)\dots (j+d+\Delta-2) (d (d+2) \dots (d+2\Delta)^{1/3}}{j(j-1)\dots (j-\Delta)} \\
    &\leq \max(C, \tilde{C})^j (d+2j)^{-3/2} \frac{(j!)^{5/6} \cdot (2j+d-2)!}{(j+d-3)!} \left(\frac{(d+2\Delta)!!}{(d-2)!!}\right)^{1/3} \frac{(j-\Delta)!}{j!}  \left(\frac{(d+2\Delta)!!}{(d+2j)!!}\right)^{3/2}
\end{align}
}
\end{proof}
}




--- ---- ---- ---- ---- 
\begin{align}
    |P_{j,\lambda}(\cos \theta) | & = \bar{P}_{j,\lambda}(1)^{-1} \sqrt{\frac{u \pi}{2}} \frac{\Gamma(\frac12 (u + \lambda)) \theta^{1/2}}{\Gamma(\frac12 (u - \lambda) + 1) \Gamma(\lambda) \sin(\theta)^\lambda} \cdot \left\{ 
|J_{\lambda-1/2}(u \theta)|\left(1 + O\left(\frac{\lambda^3}{u^2}\right) \right)\right\} \nonumber \\
& = \frac{\Gamma(j+1)\Gamma(2\lambda)}{\Gamma(j+2\lambda)} \sqrt{\frac{u \pi}{2}} \frac{\Gamma(\frac12 (u + \lambda)) \theta^{1/2}}{\Gamma(\frac12 (u - \lambda) + 1) \Gamma(\lambda) \sin(\theta)^\lambda} \cdot \left\{ 
|J_{\lambda-1/2}(u \theta)|\left(1 + O\left(\frac{\lambda^3}{u^2}\right) \right)\right\} \nonumber \\
& = \frac{\Gamma(j+1)\Gamma(2\lambda)}{\Gamma(j+2\lambda)}  \frac{\Gamma(\lambda+j/2)) }{\Gamma(j/2+1) \Gamma(\lambda) } O(j^\lambda) O(\lambda^{1/2-\lambda}) \cdot \left( O(\lambda^{-1/3}) + O\left(\frac{\lambda^{3-1/3}}{j^2}\right) \right) \nonumber \\
&\simeq \frac{j^{1/2} j^j e^{-j} \lambda^{1/2} (2\lambda)^{2\lambda-1} e^{-2\lambda+1} j^{1/2} (j/2)^{\lambda+j/2-1} e^{1-j/2-\lambda} }{j^{1/2} j^{j+2\lambda-1} e^{1-j-2\lambda}  j^{1/2} (j/2)^{j/2} e^{-j/2} \lambda^{1/2} \lambda^{\lambda-1} e^{1-\lambda}} O(j^\lambda) O(\lambda^{1/6-\lambda}) \nonumber \\
& \simeq j^{3j/2+\lambda-3j/2-2\lambda+\lambda} e^{-j-2\lambda+1+1-j/2-\lambda -1+j+2\lambda +j/2-1+\lambda} \lambda^{1/2+2\lambda-1-1/2-\lambda+1+1/6-\lambda} 2^{2\lambda-1-\lambda-j/2+1+j/2} \\
&= 
\end{align}



we have 
    \begin{equation}
        \upsilon_{j,d} \lesssim (e/2)^{-\lambda} \lambda^{1/6} \left[1 + \frac{\lambda^2}{j(j+2\lambda)} \right]^{\lambda + 1/2} ~.
    \end{equation}

From Fact \ref{fact:upsi_basicbound}, we now define 
$\delta_*=\delta_*(j,d)$ such that $m(\delta_*, j, d) = \Theta(d)$. 
Using the upper bound for $z_{j-1, d+2}^2$ from Fact \ref{fact:largestroot} we thus obtain that 
\begin{align}
    \upsilon_{j,d} &\leq \left(\frac{e_{j,\lambda}/f_{j,\lambda} - \delta_*^2 }{1-\delta_*^2} \right)^{\Theta(d)} \nonumber \\
    &= \left(\frac{(j-1)(j+2\lambda-2) - (j+\lambda-2)(j+\lambda-1)\delta_*^2 }{(j+\lambda-2)(j+\lambda-1)(1-\delta_*^2)} \right)^{\Theta(d)} \nonumber \\
    & \simeq \left(\frac{j(j+2\lambda) - (j+\lambda)^2 \delta_*^2 }{(j+\lambda)^2(1-\delta_*^2)} \right)^{\Theta(d)} \nonumber \\
    & = \left((1-\delta_*^2)^{-1} \left( 1 - \delta_*^2 - \frac{\lambda^2}{(j+\lambda)^2  }  \right)\right)^{\Theta(d)}~,
\end{align}
so if $\frac{\lambda^2}{(j+\lambda)^2} \geq  \rho (1 - \delta_*^2)  $
for $1> \rho > 0$, we obtain
\begin{equation}
    \upsilon_{j,d} \lesssim (1-\rho)^{\Theta(d)}~,
\end{equation}
as claimed. 

%$$\frac{\lambda^2}{\rho(j+\lambda)^2} =  (1 - \delta_*^2)$$
%$$\delta_*^2 = 1 - \frac{\lambda^2}{\rho(j+\lambda)^2} $$
So, it is sufficient to show that 
\begin{equation}
m\left( 1 - O\left(\frac{\lambda^2}{(j+\lambda)^2}\right) , j, \lambda\right) = \Theta(\lambda)~,     
\end{equation}
in other words, there is a (vanishingly small) fraction $\Theta(\lambda/j)$ of the roots of $\bar{P}_{j,\lambda}$ in the (vanishingly small) interval $\left[1 - O\left(\frac{\lambda^2}{(j+\lambda)^2}\right), 1 \right]$. 



For $j \gg d$, we rely on asymptotic properties of Gegenbauer polynomials. 
In particular, we consider 
\begin{theorem}[{\cite[Eq (3.4.5)]{gallardo}}]
    Let $\Lambda_\nu(x) = \frac{\Gamma(\nu+1) J_\nu(x)}{(\frac12 x)^\nu}$, where $J_\nu(x)$ is the Bessel function of the first kind, and $N = j + \lambda + \frac12$. 
    We have
    \begin{equation}
        \left(\frac{\sin \theta}{\theta} \right)^{\lambda+\frac12} P_{j,2\lambda+2}(\cos \theta) = \Lambda_\lambda( N \theta) + R_j(\theta)~,
    \end{equation}
    where $R_j(\theta) = \theta^{\frac12 - \lambda} j^{-3/2-\lambda} O_j(1)$ for $C j^{-1} \leq \theta \leq \pi - \epsilon$, and $R_j(\theta) = \theta^2 O_j(1)$ for $0 \leq \theta \leq C j^{-1}$. 
\end{theorem}

% \begin{fact}
%     For $\cos \theta_{j,d} = z_{j-1,d+2}$, we have 
%     $$\left(\frac{\sin \theta_{j,d}}{\theta_{j,d}} \right)^{\lambda+\frac12} \geq $$
%     $$|\Lambda_\lambda(N \theta_{j,d})| \leq \kappa^{-\lambda} $$
%     $$|R_j(\theta_{j,d})| \leq B \kappa^{-\lambda}  $$
% \end{fact}

\begin{corollary}[Behavior of $\upsilon_{j,d}$, large $j$ regime] Assume the Ansatz $\left(\frac{\sin \theta}{\theta} \right)^{\lambda+\frac12} P_{j,2\lambda+2}(\cos \theta) \sim \Lambda_\lambda( N \theta)$. Then 
    \begin{equation}
        \upsilon_{j,d} \lesssim (e/2)^{-\lambda} \lambda^{1/6} \left[1 + \frac{\lambda^2}{j(j+2\lambda)} \right]^{\lambda + 1/2} ~.
    \end{equation}
    In particular, if $j = \omega(\lambda)$, then there exists $\rho < 1$ such that 
    \begin{equation}
        \upsilon_{j,d} = O( \rho^{d} )~.
    \end{equation}
\end{corollary}
\begin{proof}
    The largest root of $P_{j,d}$ is given by Fact \ref{fact:largestroot}, by 
    $$z_{j,d}\leq \sqrt{\frac{(j-1)(j+d-4)}{(j+d/2-3)(j+d/2-2)}} \cos(\pi/(j+1)) := z_{j,d}^*~.$$

  Let $\cos \theta_{j,d} = z_{j-1,d+2}^*$.
From the Ansatz $\left(\frac{\sin \theta}{\theta} \right)^{\lambda+\frac12} P_{j,2\lambda+2}(\cos \theta) \sim \Lambda_\lambda( N \theta)$, and using Cauchy's asymptotic formula $J_\lambda(\lambda) \simeq \frac{\Gamma(1/3)}{2^{2/3} 3^{1/6} \pi \lambda^{1/3}}$ as well as Stirling's formula, we obtain
 \begin{align*}
    \upsilon_{j,\lambda} &= |P_{j,2\lambda+2}( \cos( \theta_{j, \lambda}) )| \\
    & \leq \left(\frac{\sin \theta_{j,d}}{\theta_{j,d}} \right)^{-\lambda-\frac12} 2^\lambda \lambda! J_\lambda\left( \theta_{j,d}(j+\lambda+1/2) \right) (\theta_{j,d}(j+\lambda+1/2))^{-\lambda} \\ 
    & \lesssim \left[\frac{(j+\lambda-2)(j+\lambda-1)}{(j-1)(j+2\lambda-2)} \right]^{\lambda + 1/2} 2^\lambda \lambda! J_\lambda( \sqrt{\lambda (\lambda-1)})  \lambda^{-\lambda} \\
    &\lesssim \left[\frac{(j+\lambda-2)(j+\lambda-1)}{(j-1)(j+2\lambda-2)} \right]^{\lambda + 1/2} \lambda^{-1/3-\lambda} 2^\lambda \lambda! \\
    & \lesssim (e/2)^{-\lambda} \lambda^{1/6} \left[1 + \frac{\lambda(\lambda-1)}{(j-1)(j+2\lambda-2)} \right]^{\lambda + 1/2}  
\end{align*}




% If we denote $C_d = \min_z J_{d/2}(z)$, and since $P_{j,\lambda}(z) > 0$ for $z > z_{j,d}$, 
% we thus have 
% \begin{align*}
%     \upsilon_{j,d} &\leq \frac{j! (d-3)!}{(j+d-3)!} \left(\frac{\sqrt{1-z_{j,d}^2}}{2}\right)^{-d/2} \left( (j+d/2)^{-d/2} \frac{\Gamma(j+d/2)}{j!} \sqrt{1-z_{j,d}^2}^{-1/2} C_{d} + O(j^{-3/2}) \right) \\
%     & = O( j^{-3d/4})~.
% \end{align*}

%
\par\noindent\rule{\textwidth}{.5pt}
\rule[.8\baselineskip]{\textwidth}{.5pt}

\clearpage


Appendix C


\begin{fact}[{\cite[Equation (2.8)]{BAI20071}}]
\label{fact:baiintegral}
\begin{equation}
\label{eq:baiintegral}
    {P}_{j, \lambda}(\cos \theta) = \frac{\Gamma(j+1) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \Gamma(\lambda+j+1/2)} \theta 2^{\lambda-1/2} \frac{1}{2\pi i} \oint_\Gamma e^{(\lambda+j)\theta z} R^{-1} \left( e^{\theta z} - \cos \theta + R e^{\theta z/2}\right)^{-\lambda+1/2} dz~,
%    \bar{P}_{j, \lambda}(\cos \theta) = \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \Gamma(\lambda+j+1/2)} \left(\frac{\theta}{2} \right)^{-\lambda+1/2} \frac{1}{2\pi i} \oint_\Gamma h(z, \theta) e^{(\lambda+j)\theta z} (z + \sqrt{z^2 +1})^{-\lambda+1/2} \frac{dz}{\sqrt{z^2+1}}~,
\end{equation}    
where $\Gamma$ is a Hankel-type loop, starting from $-\infty$, encircling both $z=\pm i$ counterclockwise, and ending at $-\infty$; and 
% $$h(z, \theta) = \left( \frac{R}{\theta \sqrt{1+z^2}} \right)^{-1}\left( \frac{(e^{\theta z /2}-e^{-\theta z/2}+ R) (e^{\theta z /2}+e^{-\theta z/2}+ R)}{2\theta (z + \sqrt{z^2+1})}\right)^{-\lambda+1/2}~,$$
% with 
$$R = \left( e^{\theta z} + e^{-\theta z} - 2\cos \theta\right)^{1/2}~.$$

\end{fact}

% \begin{theorem}[{\cite[Corollary 1]{frenzen_wong_1985}}]
% \label{theo:wong_greatbound}
%    Let $u = j + \lambda$. Then, uniformly over $0\leq \theta \leq \pi/2$, 
%    \begin{equation}
%    \label{eq:frenz}
%        \bar{P}_{j,\lambda}(\cos \theta) = \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda)\Gamma(j+1)(2u)^{\lambda-1/2}}\frac{ \theta^{1/2}}{ \sin(\theta)^\lambda }\cdot \left(J_{\lambda-1/2}(u\theta) + A_1(\theta)\frac{J_{\lambda+1/2}(u\theta)}{u} +\varepsilon(j, \lambda,\theta) \right)~,
%    \end{equation}
% where $J_\nu(z)$ is the Bessel function of the first kind, 
%    $$A_1(\theta) = (\lambda(\lambda-1))\frac{1-\theta \cot(\theta)}{2\theta}$$
%    and
%    $$|\varepsilon| \leq \frac{\theta^{\lambda+3/2}}{u^{5/2 - \lambda}}~.$$
% \end{theorem}


% \begin{theorem}[{\cite[\href{https://dlmf.nist.gov/18.15}{Eq (18.15)}]{NIST:DLMF}}]
% \label{thm:gegenbessel}
% Let $u = j + \lambda$. Then, for large $j$, 
% \begin{equation}
%       \bar{P}_{j,\lambda}(\cos \theta) = \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \sqrt{2}u^{\lambda-1/2}j! 2^\lambda} \frac{ \theta^{1/2}}{ \sin(\theta)^\lambda } \left(J_{\lambda-1/2}(u\theta) + \varepsilon(u, \theta) \right)~,
% \end{equation}
% where $J_\nu(z)$ is the Bessel function of the first kind, and
% \begin{equation}
%     \varepsilon(u, \theta) = \theta^{1/2} O_\lambda(u^{-3/2})
% \end{equation}
% for $\theta = \Omega(u^{-1})$. 
% \end{theorem} 


%from \cite{dunster2023uniform}. Concretely, we have
% \begin{proposition}[{\cite[Eq (4.4)]{dunster2023uniform}}]
% \label{prop:gegenbessel}
% Let $u = \lambda + j$ be sufficiently large. Then
%     \begin{equation}
%         \bar{P}_{j,\lambda}(\cos \theta) =  \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \sqrt{2}u^{\lambda-1/2}j! 2^\lambda}\frac{\theta^{1/2}}{\sin(\theta)^\lambda}\cdot \left\{J_{\lambda-1/2}(u \theta) \hat{A}(u, \theta) - J_{\lambda+1/2}(u\theta) \hat{B}(u, \theta) \right\}~,
%     \end{equation}
%     %     \begin{equation}
%     %     \bar{P}_{j,\lambda}(\cos \theta) = \sqrt{\frac{u \pi}{2}} \frac{\Gamma(\frac12 (u + \lambda)) }{\Gamma(\frac12 (u - \lambda) + 1) \Gamma(\lambda) } \frac{\theta^{1/2}}{\sin(\theta)^\lambda}\cdot \left\{J_{\lambda-1/2}(u \theta) \hat{A}(u, \theta) - J_{\lambda+1/2}(u\theta) \hat{B}(u, \theta) \right\}~,
%     % \end{equation}
%     where $J_\nu(z)$ is the Bessel function of the first kind, and $\hat{A}$, $\hat{B}$ admit asymptotic expansions of the form 
%     \begin{align*}
%         \hat{A}(u, \theta) & \simeq \sum_{k=0}^\infty \frac{A_k(\theta,\lambda)}{u^{2k}} ~,\\
%         \hat{B}(u, \theta) & \simeq \sum_{k=0}^\infty \frac{B_k(\theta,\lambda)}{u^{2k+1}} ~,
%     \end{align*}
%     where these expansions are uniformly valid in $0 \leq \theta \leq \pi/2$, with coefficients $A_k(\theta)$, $B_k(\theta)$ with explicit dependencies on $\lambda,\theta$. 
% \end{proposition}

Assume $j = \Theta(\lambda^\alpha)$, with $\alpha > 3/2$. 
We are interested in the above representation for  $\bar{\theta} = \arccos(z_{j-1,d+2})$. 
From Theorem \ref{thm:gegenroots_3}, we have 
$z_{j-1,d+2}^2 \geq 1 - d_{j,\lambda}/(2c_{j,\lambda})$, and thus 
$$\bar{\theta}^2 \lesssim \frac{d_{j,\lambda}}{2c_{j,\lambda}} \simeq \frac{32\lambda^2 j^4 }{16 j^6} = \frac{2\lambda^2}{j^2}~,$$
so $\bar{\theta} = O(\lambda/j)$. 
Combining this upper bound with the lower bound obtained from Fact \ref{fact:largestroot} we have $\bar{\theta} = \Theta(\lambda/j)$. 
%and in particular $\bar{\theta} = \Omega(u^{-1})$. 
In this regime, we obtain the following control 
thanks to Fact \ref{fact:baiintegral}:
\begin{lemma}
For $\theta = \Theta(\lambda/j)$ and $j = \omega(\lambda^{3/2})$, we have    
\begin{align}
  P_{j,d}(\cos \theta) & = 
\end{align}
\end{lemma}
\begin{proof}
We bound the integral in (\ref{eq:baiintegral}) by separating the tail and the region near the poles $z = \pm i$. 
We consider $0<\delta<1$ and 
\begin{align}
\Gamma = & \{ z = t \pm i \delta ; -\infty \leq t \leq -\delta\} \cup \{ z=\pm \delta + i t; -1-\delta \leq t \leq 1+\delta \} \nonumber \\
& \cup \{ z= t \pm i (1+\delta); -\delta \leq t \leq \delta\} \setminus \{z=-\delta + i t; -\delta \leq t \leq \delta\}~.    
\end{align}
Let $K>0$. We split the integration path as $\Gamma = \Gamma_{>K} \cup \Gamma_{\delta, K} \cup \Gamma_{\leq \delta}$, 
% integral as 
%     \begin{align}
%         \oint_\Gamma e^{(\lambda+j)\theta z} R^{-1} \left( e^{\theta z} - \cos \theta + R e^{\theta z/2}\right)^{-\lambda+1/2} dz &= \int_{\Gamma_{>R}} dz + \int_{\Gamma_{\leq R}} dz ~,
%     \end{align}
where $\Gamma_{>K} = \{ z \in \Gamma; |z| > K\}$, $\Gamma_{\leq \delta} = \{ z \in \Gamma; |\text{Re}(z)|\leq \delta\}$ and $\Gamma_{\delta, K} = \Gamma \setminus ( \Gamma_{>K} \cup \Gamma_{\leq \delta})$.  
Assume $K > \ln 5$. Then we obtain
\begin{align}
    |R| &= \left| e^{\theta z} + e^{-\theta z} - 2\cos \theta \right|^{1/2} \nonumber \\
    & \geq \left( e^{ -\theta \text{Re}(z)} - 2\cos \theta - e^{ \theta \text{Re}(z)}\right)^{1/2}_+ \nonumber \\
    & \geq \frac12 e^{ -\theta \text{Re}(z)}~. 
\end{align}

On the other hand, we have 
\begin{align}
    |R e^{\theta z/2}| &= \left| 1 + e^{\theta z} ( e^{\theta z} - 2\cos \theta) \right|^{1/2} \nonumber \\
    &\geq 1 - e^{\theta \text{Re}(z)}~,
\end{align}
%with $|b| \leq 2 e^{\theta \text{Re}(z)}$. 
As a result, whenever $K > \theta^{-1} \log\left(\frac{2}{1-\cos \theta} \right)$, it holds
\begin{align}
    \left| e^{\theta z} - \cos \theta + R e^{\theta z/2} \right| \geq 1 - \cos \theta - 2 e^{\theta \text{Re}(z)} \nonumber \\
    \geq \frac12 ( 1 - \cos \theta)~. 
\end{align}
By assembling these bounds, we therefore obtain
\begin{align}
\label{eq:bp1}
    \left|\int_{\Gamma_{>K}} e^{(\lambda+j)\theta z} R^{-1} \left( e^{\theta z} - \cos \theta + R e^{\theta z/2}\right)^{-\lambda+1/2} dz \right| & \leq 4 (1-\cos(\theta))^{-\lambda+1/2} \int_{\Gamma_{>K}} e^{(\lambda+j+1) \theta \text{Re}(z)} dz \nonumber \\
    & \leq 8 (1-\cos(\theta))^{-\lambda+1/2} e^{-K (\lambda+j+1)} (\lambda+j+1)^{-1} ~.
\end{align}
Since $\theta = \Theta(\lambda/j)$, picking $K \simeq \theta^{-1} \log\left(\frac{2}{1-\cos \theta} \right)$ we obtain from (\ref{eq:bp1}) 
\begin{equation}
\label{eq:vip1}
    \left|\int_{\Gamma_{>K}} e^{(\lambda+j)\theta z} R^{-1} \left( e^{\theta z} - \cos \theta + R e^{\theta z/2}\right)^{-\lambda+1/2} dz \right| \simeq \left(\frac{\lambda}{j}\right)^{-2 \lambda +1 + 2j (j+\lambda+1)/\lambda} ~. 
\end{equation}

Let us now focus on $\Gamma_{\leq \delta}$. 
In the slices $\{ z = \pm \delta + it ;  |t| \leq (1+\delta) \}$ and $\{ z = t \pm i (1+\delta);  |t| \leq \delta\}$ we have, by exploiting the monotonicity of $t \mapsto |R(z_t)|^2$, 
\begin{equation}
\label{eq:mini1}
2 \theta \delta\sin \theta \delta  \leq |R|^2 \leq  2(1-\cos \theta) + \theta^2 \delta^2~. 
\end{equation}
% Similarly, in $\{ z = t \pm i (1+\delta);  |t| \leq \delta\}$ we have 
% \begin{align}
% \label{eq:mini2}
%     \left| e^{\theta z} - \cos \theta + R e^{\theta z/2} \right| & \geq \sin (\theta \text{Im}(z)) - |R| e^{\theta \text{Re}(z)/2}  \nonumber \\
%     &\gtrsim \theta(1+\delta) - \theta^2(1+\delta^2)~,
% \end{align}
% whereas in $\{ z = \delta + i t;  |t| \leq 1+ \delta \}$ we have 
% \begin{align}
% \label{eq:mini3}
%     \left| e^{\theta z} - \cos \theta + R e^{\theta z/2} \right| & \geq e^{\delta \theta} - \cos \theta - |R| e^{\delta \theta /2} \nonumber \\
%     & \gtrsim \theta \delta - \theta^2(3/2 + \delta^2)~,
% \end{align}
% and finally in $\{ z = -\delta + i t; \delta \leq |t| \leq 1+\delta \}$ we have 
% \begin{align}
% \label{eq:mini4}
%     \left| e^{\theta z} - \cos \theta + R e^{\theta z/2} \right| & \geq | e^{\theta z} - \cos \theta| - |R| e^{-\delta \theta /2} \nonumber \\
%     & \gtrsim \sqrt{2} \theta \delta - \theta^2(1 + \delta^2)~.
% \end{align}
Similarly, we have 
\begin{align}
\label{eq:mini2}
    \left| e^{\theta z} - \cos \theta + R e^{\theta z/2} \right|  
    &\geq \theta | z + \sqrt{1 + z^2} | - o(\theta \delta) \nonumber \\
    & \gtrsim \theta \sqrt{\delta}~.
    \end{align}

Assembling (\ref{eq:mini1}) and (\ref{eq:mini2}) we obtain 
\begin{align}
\label{eq:vip2}
 \left|   \int_{\Gamma_{\leq \delta}} e^{(\lambda+j)\theta z} R^{-1} \left( e^{\theta z} - \cos \theta + R e^{\theta z/2}\right)^{-\lambda+1/2} dz \right| & \leq (2 + 4\delta) e^{(\lambda+j)\theta \delta} \theta^{-1}\delta^{-1} (\theta \sqrt{\delta})^{-\lambda + 1/2} \nonumber \\
 & \lesssim \frac{1+\delta}{\delta} e^{\lambda \delta} j \lambda^{-1} \left(\frac{\lambda \sqrt{\delta}}{j} \right)^{-\lambda + 1/2}~. 
\end{align}



Finally, we focus on $\Gamma_{\delta, K}$. We verify that $|R|$ takes its minimal value at $z=-\delta \pm i \delta$, thus $|R| \gtrsim \theta \delta$ in $\Gamma_{\delta, K}$. Similarly, $z\mapsto \left|e^{\theta z} - \cos \theta + R e^{\theta z /2} \right|$ is also monotonic for $z = t \pm i \delta$, $t \in [-K, -\delta)$, thus 
$$\left|e^{\theta z} - \cos \theta + R e^{\theta z /2} \right| \geq 1-\cos(\theta)\gtrsim \theta^2/2~.$$
Therefore, 
\begin{align}
\label{eq:vip3}
    \left| \int_{\Gamma_{\delta, K}} e^{(\lambda+j)\theta z} R^{-1} \left( e^{\theta z} - \cos \theta + R e^{\theta z/2}\right)^{-\lambda+1/2} dz \right| & \lesssim \delta^{-1} \theta^{-2\lambda} 2^{\lambda} \int_\delta^K e^{-(\lambda+j)\theta t} dt \nonumber \\
    &\lesssim \theta^{-2\lambda} 2^{\lambda} e^{-\lambda \delta} \lambda^{-1} \nonumber \\
    & \lesssim \lambda^{-2\lambda} j^{2\lambda} 2^{\lambda} e^{-\lambda \delta} \lambda^{-1} 
\end{align}
Setting $\delta = \frac12$, 


\end{proof}

% \begin{lemma}
% For $\theta = \Theta(\lambda/j)$ and $j = \omega(\lambda^{3/2})$, we have    
% \begin{align}
%     \bar{P}_{j,\lambda}(\cos \theta) &= \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \Gamma(\lambda+j+1/2)} P_{\lambda, \lambda, j}(\cos \theta) \\
%     &= \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \Gamma(\lambda+j+1/2)} \left(\frac{\theta}{2} \right)^{-\lambda+1/2} \chi(\theta, j, \lambda)~,
% \end{align}
% where 
% $\chi(\theta, j, \lambda) = O(\lambda^{-1/3})$.
% \end{lemma}
% \begin{proof}
%     \begin{align}
%   %      P_{j,d}(\theta) & = \frac{\Gamma(j+1)\Gamma(2\lambda)}{\Gamma(j+2\lambda)} \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \Gamma(\lambda+j+1/2)} \left(\frac{\theta}{2} \right)^{-\lambda+1/2} \chi(\theta, j, \lambda)
%         P_{j,d}(\theta) & = \frac{\Gamma(j+1) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \Gamma(\lambda+j+1/2)} \left(\frac{\theta}{2} \right)^{-\lambda+1/2} \chi(\theta, j, \lambda) ~,
%     \end{align}
%     so 
%     \begin{align}
%         \log P_{j,d}(\cos \theta) & \simeq -\lambda ( \log \lambda - \log j + C) + \log \chi(j,\lambda) + j \log j + \lambda \log \lambda - (2\lambda) \log \lambda - (\lambda + j) \log j \\
%         & \simeq -C \lambda + \log \chi(j, \lambda) -2 \lambda \log \lambda
%     \end{align}
% \end{proof}


% \begin{claim}
% \label{claim:besselgegen_as}
% For $\theta = \Theta(\lambda/j)$ and $j = \omega(\lambda)$, we have %, with $u = \lambda+j$, 
% \begin{equation}
% \label{eq:banan}
%     % \bar{P}_{j,\lambda}(\cos \theta) = \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \sqrt{2}u^{\lambda-1/2}j! 2^\lambda} \frac{ \theta^{1/2}}{ \sin(\theta)^\lambda } \cdot \left\{ J_{\lambda-1/2}(u \theta)\left(1 + O\left(\frac{\lambda^3}{u^2}\right) \right)\right\}~. 
%         \bar{P}_{j,\lambda}(\cos \theta) = \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) (2j)^{\lambda-1/2}\Gamma(j+1) } \frac{ \theta^{1/2}}{ \sin(\theta)^\lambda } \cdot \left\{ J_{\lambda}(\lambda)\left(1 + O\left(\frac{\lambda^3}{j^2}\right) \right)\right\}~. 
% \end{equation}
% \end{claim}


% \begin{claim}
% \label{claim:besselgegen}
% For $\theta = \Theta(\lambda/j)$, we have, with $\rho = \lambda+j$, 
% \begin{equation}
% \label{eq:banan}
%     \bar{P}_{j,\lambda}(\cos \theta) = \sqrt{\frac{u \pi}{2}} \frac{\Gamma(\frac12 (u + \lambda)) \theta^{1/2}}{\Gamma(\frac12 (u - \lambda) + 1) \Gamma(\lambda) \sin(\theta)^\lambda} \cdot \left\{ 
% J_{\lambda-1/2}(u \theta)\left(1 + O\left(\frac{\lambda^3}{u^2}\right) \right)\right\}~. 
% \end{equation}
% \end{claim}

%[Vanishing Error terms when $j = \omega(\lambda^{3/2})$]
Since $\alpha > 3/2$ and $j = \Theta(\lambda^\alpha)$, the error term in (\ref{eq:banan}) is vanishing. % when $\theta=O(\lambda/j)$. 
%Let us show how to leverage Claim \ref{claim:besselgegen} when $j = \omega(\lambda^{3/2})$. 
%From (\ref{eq:banan}), for $\theta=\Theta(\lambda/j)$ 
We have %such that $\cos \theta = z_{j-1,d+2}$, we have 
\begin{align}
    |P_{j,\lambda}(\cos \theta) | & = \bar{P}_{j,\lambda}(1)^{-1} \frac{\Gamma(2\lambda+j) \Gamma(\lambda+1/2)}{\Gamma(2\lambda) \sqrt{2}u^{\lambda-1/2}\Gamma(j+1) 2^\lambda} \frac{ \theta^{1/2}}{ \sin(\theta)^\lambda } \cdot \left\{ |J_{\lambda-1/2}(u \theta)|\left(1 + O\left(\frac{\lambda^3}{u^2}\right) \right)\right\} \nonumber \\
& =  \frac{\Gamma(\lambda+1/2)}{ \sqrt{2}u^{\lambda-1/2}2^\lambda} \frac{ \theta^{1/2}}{ \sin(\theta)^\lambda } \cdot \left\{ |J_{\lambda-1/2}(u \theta)|\left(1 + O\left(\frac{\lambda^3}{u^2}\right) \right)\right\}  \nonumber \\
& \simeq \frac{\Gamma(\lambda+1/2)}{ j^{\lambda-1/2}2^\lambda} O(j^{\lambda-1/2}) O(\lambda^{1/2-\lambda}) \cdot \left\{ O(\lambda^{-1/3}) + O\left(\frac{\lambda^{3-1/3}}{j^2}\right) \right\} \nonumber \\
& = O\left( e^{1/2-\lambda} 2^{-\lambda} \lambda^{1/6}\right) \nonumber \\
% & = \frac{\Gamma(j+1)\Gamma(2\lambda)}{\Gamma(j+2\lambda)}  \frac{\Gamma(\lambda+j/2)) }{\Gamma(j/2+1) \Gamma(\lambda) } O(j^\lambda) O(\lambda^{1/2-\lambda}) \cdot \left( O(\lambda^{-1/3}) + O\left(\frac{\lambda^{3-1/3}}{j^2}\right) \right) \nonumber \\
% &\simeq \frac{j^{1/2} j^j e^{-j} \lambda^{1/2} (2\lambda)^{2\lambda-1} e^{-2\lambda+1} j^{1/2} (j/2)^{\lambda+j/2-1} e^{1-j/2-\lambda} }{j^{1/2} j^{j+2\lambda-1} e^{1-j-2\lambda}  j^{1/2} (j/2)^{j/2} e^{-j/2} \lambda^{1/2} \lambda^{\lambda-1} e^{1-\lambda}} O(j^\lambda) O(\lambda^{1/6-\lambda}) \nonumber \\
% & \simeq j^{3j/2+\lambda-3j/2-2\lambda+\lambda} e^{-j-2\lambda+1+1-j/2-\lambda -1+j+2\lambda +j/2-1+\lambda} \lambda^{1/2+2\lambda-1-1/2-\lambda+1+1/6-\lambda} 2^{2\lambda-1-\lambda-j/2+1+j/2} \\
%&= O\left( (e/2)^{-\lambda} \lambda^{1/6} \right) \nonumber \\
&= O\left( (e/2)^{-\lambda} \right)~,
\end{align}
%\cite[Section 8.32, pg 234]{watson1922treatise}
where we have used Cauchy's asymptotic formula $J_\lambda(\lambda) \simeq \frac{\Gamma(1/3)}{2^{2/3} 3^{1/6} \pi \lambda^{1/3}}$ \cite[Section 8.2, pg 231]{watson1922treatise}, as well as Stirling's formula 
$\Gamma(x+1) \simeq \sqrt{2 \pi x} (x/e)^x$.


% \begin{proof}[Proof of Claim \ref{claim:besselgegen_as}]
% The control is a direct application of Theorem \ref{theo:wong_greatbound}. 
% In the regime $j = \omega(\lambda)$, we have
% $$\theta \cot\theta = 1 + \frac{1}{6} \frac{\lambda^2}{j^2}~,$$
% and thus
% $$A_1(\theta) = \Theta\left(\frac{\lambda^3}{j^2}\right)~.$$
% Similarly, 
% \begin{align*}
%     |\varepsilon| &\lesssim \frac{\lambda^{\lambda+3/2}}{j^{\lambda+3/2+5/2-\lambda}}
% \end{align*}
% From (\ref{eq:frenz}), we have

% \end{proof}

%\begin{proof}

%     %We denote $P_j = P_{j,d}$ by convenience.
%     Let $z_{j,d}$ be the largest root of $P_{j,d}$, and consider a given $t \leq z_{j,d}$. 
%     We consider $t_0 := \sup\{ z ; \, P_{j,d}(z)=0; z \leq t\}$ the largest root of $P_{j,d}$ below $t$. 
%     We argue inductively over $j$. 
%     Consider the Taylor decomposition of $P_{j,d}$ centered at $t_0$:
%     \begin{align}
%         P_{j,d}(t) &= \sum_{i_0=1}^j P_{j,d}^{(i_0)}(t_0) \frac{(t - t_0)^{i_0}}{i_0!}~. 
%     \end{align}
%     Now, we consider each of the terms $P_{j,d}^{(i_0)}(t_0)$ and apply again the Taylor decomposition using the same strategy. For each $i_0=1\ldots j$, consider $t_{0,i_0} = \sup\{ z; P_{j-i_0,d+2i_0}(z)=0; z \leq t_0\}$, and 
%     $$P_{j,d}^{(i_0)}(t_0) = K_{j,i_0,d} P_{j-i_0,d+2i_0}(t_0) = K_{j,i_0,d} \sum_{i_1=1}^{j-i_0} P_{j-i_0,d+2i_0}^{(i_1)}(t_{0,i_0}) \frac{(t_0-t_{0,i})^{i_1}}{i_1!}~,$$
%     where we have from Fact \ref{fact:deriv} that 
% %    $$K_{j, i, d} = \prod_{l=1}^i \frac{(j-i+1)(j-i+1 + d+2(i-1)-2)}{d+2(i-1) - 1}~. $$
%     $$K_{j, i, d} = \prod_{l=1}^i \frac{(j-i+1)(j+i+d-3)}{d+2i-3}~. $$
% Applying this Taylor decomposition recursively leads to 
% \begin{align}
%     P_{j,d}(t) &= \sum_{l=1}^{j-1} \sum_{i_0+\ldots i_l=j} \chi_{i_0, \ldots, i_l,d} \prod_{k=1}^l (t_{p(i;k-1)} - t_{p(i;k)} )^{i_k}
% \end{align}
%\end{proof}


% {\color{blue}
% *** *** *** 

% Consider a generic rotationally invariant probability measure $\mu$.  That is, for $x \sim U(S^{d-1})$ and $r \sim \nu$ independent of $x$ for some one-dimensional measure $\nu$ supported on $[0, \infty)$, we say that $\tilde{x}$ is distributed according to $\mu$ if we have the distributional equality $\tilde{x} = rx$.

% Let $\{p_i\}_{i=1}^\infty$ be the family of orthonormal polynomials with respect to $\nu$.  Then the family of functions $\{p_i \otimes P_j\}_{i,j=1}^\infty$ is orthonormal with respect to the product measure $\nu \times \omega$ where $\omega$ is the one dimensional marginal of the uniform spherical distribution, so we may decompose our link function as
% %
% \begin{align}
%     \phi(r\langle x, \theta \rangle) = \sum_{ij} \alpha_{ij} p_i(r) P_j(\langle x, \theta \rangle)
% \end{align}
% %
% For each data $x, r \in S^{d-1} \times \R_{\geq 0}$, we consider the square loss 
% %
% \begin{align}
%     \ell(\theta, x, r) := \left(\phi(r\langle x, \theta \rangle) - \phi(r\langle x, \theta^* \rangle) \right)^2,
% \end{align}
% %
% and this implies that the overall population loss loss can be written as:
% %
% \begin{align*}
%     L(\theta) &= E_{r, x}\left[\left(\phi(r\langle x, \theta \rangle) - \phi(r\langle x, \theta^* \rangle) \right)^2 \right] \\
%     &= C - 2 E_{r, x}\left[\phi(r\langle x, \theta \rangle) \phi(r\langle x, \theta^* \rangle)\right] \\
%     &= C - 2 \sum_{j} \left( \sum_{i} \alpha_{ij}^2 \right) P_{j}(\langle \theta, \theta^* \rangle)
% \end{align*}
% %
% And therefore the loss can be expressed solely as a function of the correlation $m_\theta = \langle \theta, \theta^* \rangle$. This is the reason why we will also refer to $m = m_\theta$ as the \textit{summary statistics} of the problem. Denote the corresponding function $\mathcal{L} : \R \to \R$ such that  $\mathcal{L}(m_\theta) = L(\theta)$, we have
% %
% \begin{align}
%     L'(m) = -2 \sum_{j} \left( \sum_{i} \alpha_{ij}^2 \right) P_{j}'(m)
% \end{align}


% For a fixed degree $j$, we have that $P_{j,d}'$ has $(a, j/\sqrt{d}, j-1)$ growth, with $a>0$ independent of $d$. 

% [TODO]

% Additionally, we may ask what conditions on the link function $\phi$ enable a good rate.

% Suppose $\phi(t) = \sum_k \beta_k t^k$ {\color{red} careful when we write this. is this in $L^2(\mathbb{R}, d\nu)$ ?}  Then we have

% \begin{align}
%     \alpha_{ij} &= E\left[\phi(r\langle x, \theta\rangle p_i(r) P_j(\langle x, \theta\rangle) \right] \\
%     &= \sum_k \beta_k \langle r^k, p_i(r) \rangle \langle \langle x, \theta \rangle^k, P_j(\langle x, \theta \rangle) \rangle\\
%     &= \sum_k \beta_k A_{ki} B_{kj}\\
%     &= \left[A^T D B \right]_{ij}
% \end{align}

% where $A, B$ collect correlation terms of orthogonal polynomials with monomials, and $D = diag(\beta)$.

% Therefore,

% \begin{align}
%     \sum_{i} \alpha_{ij}^2 = \|A^TDBe_j\|^2
% \end{align}

% }

%Fix $R>0$. 
% Since $\rho$ has sub-exponential tails and $\phi \in L^2(\mathbb{R}, \eta)$, we have that $\forall \epsilon>0$, there exists $R>0$ such that, uniformly over $j$ {\color{red} TODO justify this }. 
% {\color{red} instead, we first need to show that $\sum_j j^2 \beta_j < \infty$. Then focus on the bulk $j < J$, and we bound the tail $j > J$ separately}. 
% \begin{align}
%     \int_0^R \rho(dr) \bar{\alpha}^2_{j,r,d} &\geq (1-\epsilon) \beta_{j,d}~.
% %    \beta_{j,d} &= \mathbb{E}_{\rho} [\bar{\alpha}_{j,r,d}^2]
% \end{align}
% It follows that 
% \begin{align}
%    \mathbb{E}_\rho \left[r^{-1}  \bar{\alpha}_{j,d,r}^2 \right] &\geq \int_0^R r^{-1}  \bar{\alpha}_{j,d,r}^2 \rho(dr) \nonumber \\
%    &\geq R^{-1} \int_0^R   \bar{\alpha}_{j,d,r}^2 \rho(dr) \nonumber \\
%    &\geq R^{-1} (1-\epsilon) \beta_{j,d}~,
% %   &\geq \frac{1}{N(j,d)  \| P_{j,d}\|^{4}} 
% %   \mathbb{E}_\rho \left[r^{-1}  \bar{\alpha}_{j,d,r}^2 \right] &= \frac{1}{N(j,d)  \| P_{j,d}\|^{4}} \int_{0}^\infty \rho(dr) r^{-1} [\langle \phi^{(r)}, P_j \rangle_{u_d}]^2 \nonumber \\
%  %  &\geq \frac{1}{N(j,d)  \| P_{j,d}\|^{4}} 
% \end{align}
